It's All Around You: Range-Guided Cylindrical Network for 3D Object Detection

Modern perception systems in the field of autonomous driving rely on 3D data analysis. LiDAR sensors are frequently used to acquire such data due to their increased resilience to different lighting conditions. Although rotating LiDAR scanners produce ring-shaped patterns in space, most networks analyze their data using an orthogonal voxel sampling strategy. This work presents a novel approach for analyzing 3D data produced by 360-degree depth scanners, utilizing a more suitable coordinate system, which is aligned with the scanning pattern. Furthermore, we introduce a novel notion of range-guided convolutions, adapting the receptive field by distance from the ego vehicle and the object's scale. Our network demonstrates powerful results on the nuScenes challenge, comparable to current state-of-the-art architectures. The backbone architecture introduced in this work can be easily integrated onto other pipelines as well.

==> Images/tables/ablation.tex <==

\begin{table*}[!t]
\centering
% \begin{center}
\begin{tabular}{l cccc cccc} % \hspace*{} for Left-right shift of the entire table
\toprule

\textbf{Method} & \textit{mAP} & \textit{mATE} & \textit{mASE} & \textit{mAOE} & \textit{mAVE} & \textit{mAAE} & \textit{NDS} \\
	

\midrule            
w/o guide, w/o CC. mod. 
& - & - & - & - & - & - & - \\
w/\space\space\space guide, w/o CC. mod. 
& - & - & - & - & - & - & - \\
w/o guide, w/\space\space\space CC. mod. 
& - & - & - & - & - & - & - \\
w/\space\space\space guide, w/\space\space\space CC. mod. 
& - & - & - & - & - & - & - \\
\midrule            

%& 0.5705 & 0.2830 
%& 0.2520 & 0.2917
%& 0.2690 & 0.1726
%& 0.6584 \\
\end{tabular}
% \end{center}
\vspace{0.08cm}		
\caption{ {\bf  Ablation Experiment on nuScenes Validation set:} Cylindrical-coordinate modifications (CC. mod.) refers to modification explained on subsection Multi Group Center Head under section Method for both orientation and velocity.
}
\vspace{-0.1cm}
\label{tables:ablation}
\end{table*}


==> Images/tables/ablation_cls_orient.tex <==


\begin{table*}[!t]
\centering
% \begin{center}
\begin{tabular}{l c c c c c c c c c| c | c |} % \hspace*{} for Left-right shift of the entire table
\toprule

%\textbf{Method} & \textit{Car} & \textit{Truck} & \textit{Bus} & \textit{Trailer} & \textit{CV} & \textit{Ped} & \textit{Motor}  & \textit{Bicycle} & \textit{TC} & \textit{Barrier} \\
	
\textbf{Method} & \textit{Car} & \textit{Truck} & \textit{Bus} & \textit{Trailer} & \textit{CV} & \textit{Ped} & \textit{Motor}  & \textit{Bicycle} & \textit{Barrier} & \textit{mAOE} & \textit{mAP(2m)}\\	

\midrule            
w/o CC. mod.
& 0.105 & 0.102 & 0.076 & \textbf{0.500} & 0.968 & 0.376 & 0.281  & \textbf{0.322}  & 0.096 & 0.314 & 0.618\\
w/\space\space\space CC. mod.
& \textbf{0.087} & \textbf{0.058} & \textbf{0.041} & 0.529 & \textbf{0.859} & \textbf{0.354} & \textbf{0.251}  & 0.357  & \textbf{0.083} & \textbf{0.291} & \textbf{0.623}\\

\midrule            

%& 0.5705 & 0.2830 
%& 0.2520 & 0.2917
%& 0.2690 & 0.1726
%& 0.6584 \\
\end{tabular}
% \end{center}
\vspace{0.08cm}		
\caption{ {\bf  Ablation Experiment on nuScenes Validation set for mAOE (mean average Orientation Error), calculated for all the detected objects  under 2m distance in between two centers by the nuScenes challenge rules:} Cylindrical-coordinate modifications (CC. mod.) refers to modification explained on subsection Multi Group Center Head under section Method for both orientation and velocity. Even though Traffic cones do not have orientation estimation.
}
\vspace{-0.1cm}
\label{tables:ablation_v}
\end{table*}



==> Images/tables/ablation_cls_velo.tex <==

\begin{table*}[!t]
\centering
% \begin{center}
\begin{tabular}{l c c c c c c c c | c | c |} % \hspace*{} for Left-right shift of the entire table
\toprule

%\textbf{Method} & \textit{Car} & \textit{Truck} & \textit{Bus} & \textit{Trailer} & \textit{CV} & \textit{Ped} & \textit{Motor}  & \textit{Bicycle} & \textit{TC} & \textit{Barrier} \\
	
\textbf{Method} & \textit{Car} & \textit{Truck} & \textit{Bus} & \textit{Trailer} & \textit{CV} & \textit{Ped} & \textit{Motor}  & \textit{Bicycle} & \textit{mAVE} & \textit{mAP(2m)}\\	

\midrule            
w/o CC. mod.
& 0.292 & 0.294 & 0.532 & 0.210 & \textbf{0.128} & 0.241 & 0.578 & 0.221  & 0.312 & 0.618\\

w/\space\space\space CC. mod.
& \textbf{0.262} & \textbf{0.257} & \textbf{0.445} &  \textbf{0.180} & 0.133 & \textbf{0.205}  & \textbf{0.465}  & \textbf{0.200} & \textbf{0.268} & \textbf{0.623} \\

\midrule            

\end{tabular}
% \end{center}
\vspace{0.08cm}		
\caption{ {\bf  Ablation Experiment on nuScenes Validation set for mAVE (mean average Velocity Error):} Cylindrical-coordinate modifications (CC. mod.) refers to modification explained on subsection Multi Group Center Head under section Method for both orientation and velocity.  CV stands for Construction Vehicle, Ped for Pedestrian and Motor for Motorcycle. Traffic cones and barriers do not have velocity estimation.
}
\vspace{-0.1cm}
\label{tables:ablation}
\end{table*}




0.294
0.532
0.210
0.128
0.241
0.578
0.221


==> Images/tables/ablation_short.tex <==

\begin{table}[!t]
\centering
% \begin{center}
\begin{tabular}{l cccc cccc} % \hspace*{} for Left-right shift of the entire table
\toprule

\textbf{Method} & \textit{mAP} & \textit{NDS} \\
	

\midrule            
w/o guide, w/o CC. mod. 
& - & - \\
w/\space\space\space guide, w/o CC. mod. 
& - & - \\
w/o guide, w/\space\space\space CC. mod. 
& - & - \\
w/\space\space\space guide, w/\space\space\space CC. mod. 
& - & - \\
\midrule            

%& 0.5705 & 0.2830 
%& 0.2520 & 0.2917
%& 0.2690 & 0.1726
%& 0.6584 \\
\end{tabular}
% \end{center}
\vspace{0.08cm}		
\caption{ {\bf Ablation Experiment on nuScenes Validation set:} Cylindrical-coordinate modifications (CC. mod.) refers to modification explained on subsection Multi Group Center Head under section Method. 
}
\vspace{-0.3cm}
\label{tables:ablation}
\end{table}	

==> Images/tables/ablation_short_guided.tex <==

\begin{table}[!t]
\centering
% \begin{center}
\begin{tabular}{l cccc cccc} % \hspace*{} for Left-right shift of the entire table
\toprule

\textbf{Method} & \textit{mAP} & \textit{NDS} \\
	

\midrule            

w/o range-guided backbone
& - & - \\
w/\space\space\space range-guided backbone 
& - & - \\
\midrule            

%& 0.5705 & 0.2830 
%& 0.2520 & 0.2917
%& 0.2690 & 0.1726
%& 0.6584 \\
\end{tabular}
% \end{center}
\vspace{0.08cm}		
\caption{ {\bf Ablation Experiment on nuScenes Validation set for the range-guided backbone.} 
}
\vspace{-0.3cm}
\label{tables:ablation_guide}
\end{table}	

==> Images/tables/ablation_velo_orient.tex <==




\begin{table*}[!t]
\centering
% \begin{center}
\begin{tabular}{|l |c |c c c c c c c c c| c | c |} % \hspace*{} for Left-right shift of the entire table
\toprule

%\textbf{Method} & \textit{Car} & \textit{Truck} & \textit{Bus} & \textit{Trailer} & \textit{CV} & \textit{Ped} & \textit{Motor}  & \textit{Bicycle} & \textit{TC} & \textit{Barrier} \\
	
\textbf{Error} & \textbf{CCm.} & \textit{Car} & \textit{Truck} & \textit{Bus} & \textit{Trailer} & \textit{CV} & \textit{Ped} & \textit{Motor}  & \textit{Bicycle} & \textit{Barrier} & \textit{mAE} & \textit{mAP(2m)}\\	

\midrule            
\multirow{2}{*}{Velo.} & X
& 0.292 & 0.294 & 0.532 & 0.210 & \textbf{0.128} & 0.241 & 0.578 & 0.221  & - & 0.312 & 0.618\\
\multirow{2}{*}{} & V
& \textbf{0.262} & \textbf{0.257} & \textbf{0.445} &  \textbf{0.180} & 0.133 & \textbf{0.205}  & \textbf{0.465}  & \textbf{0.200} & - & \textbf{0.268} & \textbf{0.623}\\

\midrule            
\multirow{2}{*}{Orient.} & X & 0.105 & 0.102 & 0.076 & \textbf{0.500} & 0.968 & 0.376 & 0.281  & \textbf{0.322}  & 0.096 & 0.314 & 0.618\\
\multirow{2}{*}{} & V
& \textbf{0.087} & \textbf{0.058} & \textbf{0.041} & 0.529 & \textbf{0.859} & \textbf{0.354} & \textbf{0.251}  & 0.357  & \textbf{0.083} & \textbf{0.291} & \textbf{0.623}\\
\midrule
%& 0.5705 & 0.2830 
%& 0.2520 & 0.2917
%& 0.2690 & 0.1726
%& 0.6584 \\
\end{tabular}
% \end{center}
\vspace{0.08cm}		
\caption{ {\bf  Ablation Experiment on nuScenes Validation set for mAVE and mAOE (mean average Velocity / Orientation Error):} By nuScenes rules the error is calculated for all the detected objects  under 2m distance in between two centers (GT and predicted). Meaning, higher mAP means more detected objects to calculate error for. Cylindrical-coordinate modifications (CCm.) refers to modification explained on subsection Multi Group Center Head under section Method for both orientation and velocity. Barrier do not have velocity estimation and traffic cones do not have both (orientation and velocity).
}
\vspace{-0.1cm}
\label{tables:ablation_v}
\end{table*}



==> Images/tables/ablation_velo_orient_short.tex <==





\begin{table}[!t]
\centering
% \begin{center}
\begin{tabular}{|c |c | c| c | c |} % \hspace*{} for Left-right shift of the entire table
\toprule

%\textbf{Method} & \textit{Car} & \textit{Truck} & \textit{Bus} & \textit{Trailer} & \textit{CV} & \textit{Ped} & \textit{Motor}  & \textit{Bicycle} & \textit{TC} & \textit{Barrier} \\
	
\textbf{CC. mod.} & \textit{mAOE} & \textit{mAVE} & \textit{mAP} & \textit{NDS} \\	

\midrule 
X & 0.314 & 0.312 & 0.574 & 0.652\\
V & \textbf{0.268} & \textbf{0.291} & \textbf{0.577} & \textbf{0.661}\\


\midrule
%& 0.5705 & 0.2830 
%& 0.2520 & 0.2917
%& 0.2690 & 0.1726
%& 0.6584 \\
\end{tabular}
% \end{center}
\vspace{0.08cm}		
\caption{ {\bf  Ablation Experiment on nuScenes Validation set for mAVE and mAOE (mean average Velocity / Orientation Error):} By nuScenes rules the error is calculated for all the detected objects  under 2m distance in between two centers (GT and predicted). Meaning, higher mAP means more detected objects to calculate error for. Cylindrical-coordinate modifications (CCm.) refers to modification explained on subsection Multi Group Center Head under section Method for both orientation and velocity.
}
\vspace{-0.1cm}
\label{tables:ablation_v}
\end{table}



==> Images/tables/test_result.tex <==

\begin{table*}[!t]
\vspace{0.18cm}
\centering
% \begin{center}
\begin{tabular}{l cccc cccc} % \hspace*{} for Left-right shift of the entire table
\toprule

\textbf{Method} & \textit{mAP} & \textit{mATE} & \textit{mASE} & \textit{mAOE} & \textit{mAVE} & \textit{mAAE} & \textit{NDS} \\
	

\midrule            
CBGS \cite{cbgs} 
& 0.528
& 0.300
& 0.247
& 0.379
& 0.245
& 0.140
& 0.633 \\
CVCNet single
& 0.558
& 0.300
& 0.248
& 0.431
& 0.269
& 0.119
& 0.642 \\
CVCNet single V2
& 0.553
& 0.300
& 0.244
& 0.389
& 0.268
& 0.122
& 0.644 \\
MMDetection3D \cite{mmdetection}
& 0.575
& 0.316
& 0.256
& 0.409
& 0.236
& 0.124
& 0.653 \\
HotSpotNet-0.1m \cite{hotspot}
& 0.593
& 0.274
& 0.239
& 0.384
& 0.333
& 0.133
& 0.660 \\
CenterPoint single\cite{centerpoint}
& 0.603 
& 0.262
& 0.239
& 0.361
& 0.288
& 0.136
& 0.673 \\
Ours
& 0.584
& 0.272
& 0.243
& 0.382
& 0.293
& 0.126
& 0.661 \\
\midrule            

%& 0.5705 & 0.2830 
%& 0.2520 & 0.2917
%& 0.2690 & 0.1726
%& 0.6584 \\
\end{tabular}
% \end{center}
\vspace{0.08cm}		
\caption{ {\bf nuScenes Experiment Results on Test set:} Top results for \textit{single model} on the LiDAR track, taken from the nuScenes website.} 

%\vspace{0.1cm}
\label{tables:test results}
\end{table*}	

==> macros.tex <==
\long\def\ignorethis#1{}

% colors
\usepackage{color}
\definecolor{gray}{rgb}{0.35,0.35,0.35}
\definecolor{red}{rgb}{1,0,0}
\definecolor{dark-green}{rgb}{0,0.4,0}
\definecolor{dark-pink}{rgb}{0.78,0.08,0.52}
\definecolor{blue}{rgb}{0,0,1}
\definecolor{orange}{rgb}{1,0.55,0}
\definecolor{white}{rgb}{1,1,1}
\definecolor{black}{rgb}{1,1,1}
\definecolor{dark-brown}{rgb}{0.2,0.1,0}


\newcommand{\todo}[1]{{\color{red}TODO: #1}\normalfont}
\newcommand{\Meytal}[1]{{\color{dark-green}Meytal: #1}\normalfont}
\newcommand{\Dan}[1]{{\color{orange}Dan: #1}\normalfont}
\newcommand{\add}[1]{{\color{blue}add!#1}\normalfont}
%%% comment \ShowNotes out to remove all colored comments defined with \newcommand below %%%
% \newcommand*{\ShowNotes}{}

\ifdefined\ShowNotes
\newcommand{\whitetxt}[1]{{\color{white}#1}\normalfont}

\newcommand{\jbox}[2]{
  \fbox{%
  \begin{minipage}{#1}%
  \hfill\vspace{#2}%
  \end{minipage}%
  }}
\else
  \newcommand{\colornote}[3]{}
\fi
% colored comments



% subfigures with automatic width
\newbox\jsavebox
\newcommand{\jsubfig}[2]{%
\sbox\jsavebox{#1}%
\parbox[t]{\wd\jsavebox}{\centering\usebox\jsavebox\\#2}%
}

\newcommand{\jcell}[1]{%
  {%
 \renewcommand{\arraystretch}{0}%
 \begin{tabular}{@{}c@{}}%
#1%
\end{tabular}%
}}
